Sim-on-Wheels: Physical World in the Loop Simulation for Self-Driving

We present Sim-on-Wheels, a safe, realistic, and vehicle-in-loop framework to test autonomous vehicles' performance in the real world under safety-critical scenarios. Sim-on-wheels runs on a self-driving vehicle operating in the physical world. It creates virtual traffic participants with risky behaviors and seamlessly inserts the virtual events into images perceived from the physical world in real-time. The manipulated images are fed into autonomy, allowing the self-driving vehicle to react to such virtual events. The full pipeline runs on the actual vehicle and interacts with the physical world, but the safety-critical events it sees are virtual. Sim-on-Wheels is safe, interactive, realistic, and easy to use. The experiments demonstrate the potential of Sim-on-Wheels to facilitate the process of testing autonomous driving in challenging real-world scenes with high fidelity and low risk.

==> 06-discussion.tex <==
\section{Certifiable Evaluation using HIL}

\todo{Shenlong}
In this section, we address the critical question of how to trust the performance evaluation in simulation. Specifically, we ask whether it is possible to obtain a certificate of real-world autonomy under specific scenarios based on the corresponding hardware-in-the-loop simulation performance. To the best of our knowledge, no prior self-driving simulators have been able to provide this level of certainty. This is due to two main challenges: (1) a significant gap between reality and simulation exists across various stages in the simulator, including sensor simulation, dynamics simulation, and mechanical components simulation; (2) there is a lack of a mathematical toolkit to quantify and analyze how this gap is propagated from sensing to actions.

Our proposed novel simulation protocol can effectively overcome the aforementioned challenges. Firstly, the hardware-in-the-loop simulation system is based on physical systems involving real-world vehicles, computing devices, and real sensory data. The only gap between reality and simulation exists in the inserted objects, which greatly reduces the domain gap and minimizes the discrepancy between autonomy behaviors in real and simulated scenarios. Additionally, inspired by recent research on certifying robustness to adversarial examples, we can use Lipschitz's constant estimation to analyze the certified $\ell_p$-norm ball of our autonomy module. Suppose the gap between simulation and reality in a given scenario is upper-bounded by $\epsilon$, and the autonomy module's predicted action is $\by$. In that case, we can obtain a certificate that the module's action in the real world, in terms of speed profile, is guaranteed to be within an $\ell_2$-norm ball centered at $\by$ with a radius of $L \cdot \epsilon$ where $L$ is the Lipschitz constant of the autonomy module. Note that the tighter ball or a $\ell_p$-norm ball can be estimated by formulating this question into the following optimization question. \shenlongsay{TODO: we need to provide detailed math on how to estimate the size of the ball}


